ElasticTTT: Prior-Preserving Test-Time Tuning for Video Editing

Test-Time Tuning (TTT) on pretrained diffusion models has emerged as a powerful paradigm for video editing. However, there exists a foundational mismatch between the distribution-mapping nature of generative models and the single-point optimization of standard TTT. In this paper, we demonstrate that this mismatch triggers \textit{Prior Collapse}, a degenerate state where the model discards the text conditions and spatial latents, collapsing generations to the source video, or entangling the features of distinct regions. To resolve this, we propose \textbf{ElasticTTT}, a novel framework that preserves the prior generative distribution and rescues generative elasticity. Specifically, we propose \textit{Target Distribution Regularization} to prevent sharp memorization minima, \textit{Contrastive CFG} to guide inference away from source biases, and \textit{Asynchronous Noise Schedule} to preserve unedited regions. Extensive evaluations, supported by theoretical analysis, demonstrate that ElasticTTT successfully preserves the generative prior of the base model, achieving state-of-the-art performance on one-shot video editing.

==> 1 <==
FROM hub.byted.org/base/lab.cuda.devel:12.8.0

ENV http_proxy="http://sys-proxy-rd-relay.byted.org:8118"
ENV https_proxy="http://sys-proxy-rd-relay.byted.org:8118"
ENV no_proxy="byted.org"
ENV PYENV_VERSION 3.13.11
ENV PYENV_ROOT /home/tiger/.pyenv
ENV PATH $PYENV_ROOT/shims:$PYENV_ROOT/bin:$PATH

RUN apt-get update && apt-get install -y \
    make build-essential libssl-dev zlib1g-dev \
    libbz2-dev libreadline-dev libsqlite3-dev curl git \
    libncursesw5-dev xz-utils tk-dev libxml2-dev libxmlsec1-dev libffi-dev liblzma-dev \
    && rm -rf /var/lib/apt/lists/*

RUN curl https://pyenv.run | bash \
    && pyenv install $PYENV_VERSION \
    && pyenv global $PYENV_VERSION \
    && pyenv rehash \
    && chown -R 1000:1000 $PYENV_ROOT

RUN /home/tiger/.pyenv/shims/python3 -m pip install uv

ENV NVIDIA_TF32_OVERRIDE 0

# Step 1: Install PyTorch and all standard dependencies
RUN if [ "${REGION}" == "china-north-lf" ]; then \
        export http_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export https_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export no_proxy="byted.org" && \
        echo "set proxy -> http_proxy=${http_proxy}"; \
    else \
        echo "no proxy is needed" ; \
    fi && \
    pip3 install --no-cache-dir --upgrade pip setuptools wheel && \
    pip3 install --no-cache-dir torch==2.11.0 torchvision==0.26.0 torchaudio==2.11.0 --index-url https://download.pytorch.org/whl/cu128 && \
    pip3 install --no-cache-dir --pre torchcodec --index-url https://download.pytorch.org/whl/nightly/cu128 && \
    pip3 install --no-cache-dir ninja packaging
    
# Step 2: Install flash-attn separately so it recognizes the fully installed Torch environment
RUN if [ "${REGION}" == "china-north-lf" ]; then \
        export http_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export https_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export no_proxy="byted.org"; \
    fi && \
    MAX_JOBS=128 pip3 install --no-cache-dir flash-attn

RUN if [ "${REGION}" == "china-north-lf" ]; then \
        export http_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export https_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export no_proxy="byted.org"; \
    fi && \
    pip3 install absl-py==2.4.0 && \
    pip3 install accelerate==1.13.0 && \
    pip3 install addict==2.4.0 && \
    pip3 install anyio==4.12.1 && \
    pip3 install argbind==0.3.9 && \
    pip3 install asttokens==3.0.1 && \
    pip3 install audioread==3.1.0 && \
    pip3 install bitsandbytes==0.49.2 && \
    pip3 install byted-wandb==0.13.94 && \
    pip3 install bytedance-metrics==0.5.2 && \
    pip3 install bytedbackgrounds==0.0.6 && \
    pip3 install byteddatabus==1.0.8 && \
    pip3 install byteddps==0.1.3 && \
    pip3 install bytedenv==0.7.3 && \
    pip3 install bytedmemfd==0.2 && \
    pip3 install bytedmetrics==0.11.0 && \
    pip3 install bytedztijwthelper==0.0.24 && \
    pip3 install bytedztispiffe==0.0.17 && \
    pip3 install certifi==2026.2.25 && \
    pip3 install cffi==2.0.0 && \
    pip3 install charset-normalizer==3.4.6 && \
    pip3 install click==8.3.1 && \
    pip3 install contourpy==1.3.3 && \
    pip3 install cryptography==46.0.5 && \
    pip3 install cycler==0.12.1 && \
    pip3 install decorator==5.2.1 && \
    pip3 install Deprecated==1.3.1 && \
    pip3 install descript-audiotools==0.7.2 && \
    pip3 install diffusers==0.37.0 && \
    pip3 install docker-pycreds==0.4.0 && \
    pip3 install docstring_parser==0.17.0 && \
    pip3 install einops==0.8.2 && \
    pip3 install executing==2.2.1 && \
    pip3 install ffmpeg==1.4 && \
    pip3 install ffmpy==1.0.0 && \
    pip3 install filelock==3.25.2 && \
    pip3 install fire==0.7.1 && \
    pip3 install flatten-dict==0.4.2 && \
    pip3 install fonttools==4.62.1 && \
    pip3 install fsspec==2026.2.0 && \
    pip3 install ftfy==6.3.1 && \
    pip3 install gitdb==4.0.12 && \
    pip3 install GitPython==3.1.46 && \
    pip3 install grpcio==1.78.0 && \
    pip3 install h11==0.16.0 && \
    pip3 install hf-xet==1.4.2 && \
    pip3 install httpcore==1.0.9 && \
    pip3 install httpx==0.28.1 && \
    pip3 install huggingface_hub==0.36.2 && \
    pip3 install idna==3.11 && \
    pip3 install ImageIO==2.37.3 && \
    pip3 install imageio-ffmpeg==0.6.0 && \
    pip3 install importlib_metadata==9.0.0 && \
    pip3 install importlib_resources==6.5.2 && \
    pip3 install ipaddress==1.0.23 && \
    pip3 install ipython==9.11.0 && \
    pip3 install ipython_pygments_lexers==1.1.1 && \
    pip3 install jedi==0.19.2 && \
    pip3 install Jinja2==3.1.6 && \
    pip3 install joblib==1.5.3 && \
    pip3 install julius==0.2.7 && \
    pip3 install kiwisolver==1.5.0 && \
    pip3 install lazy-loader==0.5 && \
    pip3 install librosa==0.11.0 && \
    pip3 install llvmlite==0.46.0 && \
    pip3 install Markdown==3.10.2 && \
    pip3 install markdown-it-py==4.0.0 && \
    pip3 install markdown2==2.5.5 && \
    pip3 install MarkupSafe==3.0.3 && \
    pip3 install matplotlib==3.10.8 && \
    pip3 install matplotlib-inline==0.2.1 && \
    pip3 install mdurl==0.1.2 && \
    pip3 install mmengine==0.10.7 && \
    pip3 install mova==0.1.0 && \
    pip3 install mpmath==1.3.0 && \
    pip3 install msgpack==1.0.8 && \
    pip3 install networkx==3.6.1 && \
    pip3 install ninja==1.13.0 && \
    pip3 install numba==0.64.0 && \
    pip3 install numpy==2.4.3 && \
    pip3 install opencv-python==4.13.0.92 && \
    pip3 install parso==0.8.6 && \
    pip3 install pexpect==4.9.0 && \
    pip3 install pillow==12.1.1 && \
    pip3 install platformdirs==4.9.4 && \
    pip3 install pooch==1.9.0 && \
    pip3 install promise==2.3 && \
    pip3 install prompt_toolkit==3.0.52 && \
    pip3 install protobuf==3.19.6 && \
    pip3 install psutil==7.2.2 && \
    pip3 install ptyprocess==0.7.0 && \
    pip3 install pure_eval==0.2.3 && \
    pip3 install pycparser==3.0 && \
    pip3 install Pygments==2.19.2 && \
    pip3 install PyJWT==2.12.1 && \
    pip3 install pyloudnorm==0.2.0 && \
    pip3 install pyOpenSSL==26.0.0 && \
    pip3 install pyparsing==3.3.2 && \
    pip3 install pystoi==0.4.1 && \
    pip3 install python-dateutil==2.9.0.post0 && \
    pip3 install PyYAML==6.0.3 && \
    pip3 install randomname==0.2.1 && \
    pip3 install regex==2026.2.28 && \
    pip3 install requests==2.32.5 && \
    pip3 install rich==14.3.3 && \
    pip3 install safetensors==0.7.0 && \
    pip3 install schedule==1.2.2 && \
    pip3 install scikit-learn==1.8.0 && \
    pip3 install scipy==1.17.1 && \
    pip3 install sentry-sdk==2.56.0 && \
    pip3 install setproctitle==1.3.7 && \
    pip3 install setuptools==80.10.2 && \
    pip3 install shortuuid==1.0.13 && \
    pip3 install six==1.17.0 && \
    pip3 install smmap==5.0.3 && \
    pip3 install soundfile==0.13.1 && \
    pip3 install soxr==1.0.0 && \
    pip3 install stack-data==0.6.3 && \
    pip3 install sympy==1.14.0 && \
    pip3 install tensorboard==2.20.0 && \
    pip3 install tensorboard-data-server==0.7.2 && \
    pip3 install termcolor==3.3.0 && \
    pip3 install threadpoolctl==3.6.0 && \
    pip3 install tokenizers==0.22.2 && \
    pip3 install tqdm==4.67.3 && \
    pip3 install traitlets==5.14.3 && \
    pip3 install transformers==4.57.6 && \
    pip3 install triton==3.6.0 && \
    pip3 install typing_extensions==4.15.0 && \
    pip3 install urllib3==1.26.20 && \
    pip3 install wcwidth==0.6.0 && \
    pip3 install Werkzeug==3.1.7 && \
    pip3 install wheel==0.46.3 && \
    pip3 install wrapt==2.1.2 && \
    pip3 install yapf==0.43.0 && \
    pip3 install yunchang==0.6.4 && \
    pip3 install zipp==3.23.0


==> arxiv_meow-2/1 <==
FROM hub.byted.org/base/lab.cuda.devel:12.8.0

ENV http_proxy="http://sys-proxy-rd-relay.byted.org:8118"
ENV https_proxy="http://sys-proxy-rd-relay.byted.org:8118"
ENV no_proxy="byted.org"
ENV PYENV_VERSION 3.13.11
ENV PYENV_ROOT /home/tiger/.pyenv
ENV PATH $PYENV_ROOT/shims:$PYENV_ROOT/bin:$PATH

RUN apt-get update && apt-get install -y \
    make build-essential libssl-dev zlib1g-dev \
    libbz2-dev libreadline-dev libsqlite3-dev curl git \
    libncursesw5-dev xz-utils tk-dev libxml2-dev libxmlsec1-dev libffi-dev liblzma-dev \
    && rm -rf /var/lib/apt/lists/*

RUN curl https://pyenv.run | bash \
    && pyenv install $PYENV_VERSION \
    && pyenv global $PYENV_VERSION \
    && pyenv rehash \
    && chown -R 1000:1000 $PYENV_ROOT

RUN /home/tiger/.pyenv/shims/python3 -m pip install uv

ENV NVIDIA_TF32_OVERRIDE 0

# Step 1: Install PyTorch and all standard dependencies
RUN if [ "${REGION}" == "china-north-lf" ]; then \
        export http_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export https_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export no_proxy="byted.org" && \
        echo "set proxy -> http_proxy=${http_proxy}"; \
    else \
        echo "no proxy is needed" ; \
    fi && \
    pip3 install --no-cache-dir --upgrade pip setuptools wheel && \
    pip3 install --no-cache-dir torch==2.11.0 torchvision==0.26.0 torchaudio==2.11.0 --index-url https://download.pytorch.org/whl/cu128 && \
    pip3 install --no-cache-dir --pre torchcodec --index-url https://download.pytorch.org/whl/nightly/cu128 && \
    pip3 install --no-cache-dir ninja packaging
    
# Step 2: Install flash-attn separately so it recognizes the fully installed Torch environment
RUN if [ "${REGION}" == "china-north-lf" ]; then \
        export http_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export https_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export no_proxy="byted.org"; \
    fi && \
    MAX_JOBS=128 pip3 install --no-cache-dir flash-attn

RUN if [ "${REGION}" == "china-north-lf" ]; then \
        export http_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export https_proxy="http://sys-proxy-rd-relay.byted.org:8118" && \
        export no_proxy="byted.org"; \
    fi && \
    pip3 install absl-py==2.4.0 && \
    pip3 install accelerate==1.13.0 && \
    pip3 install addict==2.4.0 && \
    pip3 install anyio==4.12.1 && \
    pip3 install argbind==0.3.9 && \
    pip3 install asttokens==3.0.1 && \
    pip3 install audioread==3.1.0 && \
    pip3 install bitsandbytes==0.49.2 && \
    pip3 install byted-wandb==0.13.94 && \
    pip3 install bytedance-metrics==0.5.2 && \
    pip3 install bytedbackgrounds==0.0.6 && \
    pip3 install byteddatabus==1.0.8 && \
    pip3 install byteddps==0.1.3 && \
    pip3 install bytedenv==0.7.3 && \
    pip3 install bytedmemfd==0.2 && \
    pip3 install bytedmetrics==0.11.0 && \
    pip3 install bytedztijwthelper==0.0.24 && \
    pip3 install bytedztispiffe==0.0.17 && \
    pip3 install certifi==2026.2.25 && \
    pip3 install cffi==2.0.0 && \
    pip3 install charset-normalizer==3.4.6 && \
    pip3 install click==8.3.1 && \
    pip3 install contourpy==1.3.3 && \
    pip3 install cryptography==46.0.5 && \
    pip3 install cycler==0.12.1 && \
    pip3 install decorator==5.2.1 && \
    pip3 install Deprecated==1.3.1 && \
    pip3 install descript-audiotools==0.7.2 && \
    pip3 install diffusers==0.37.0 && \
    pip3 install docker-pycreds==0.4.0 && \
    pip3 install docstring_parser==0.17.0 && \
    pip3 install einops==0.8.2 && \
    pip3 install executing==2.2.1 && \
    pip3 install ffmpeg==1.4 && \
    pip3 install ffmpy==1.0.0 && \
    pip3 install filelock==3.25.2 && \
    pip3 install fire==0.7.1 && \
    pip3 install flatten-dict==0.4.2 && \
    pip3 install fonttools==4.62.1 && \
    pip3 install fsspec==2026.2.0 && \
    pip3 install ftfy==6.3.1 && \
    pip3 install gitdb==4.0.12 && \
    pip3 install GitPython==3.1.46 && \
    pip3 install grpcio==1.78.0 && \
    pip3 install h11==0.16.0 && \
    pip3 install hf-xet==1.4.2 && \
    pip3 install httpcore==1.0.9 && \
    pip3 install httpx==0.28.1 && \
    pip3 install huggingface_hub==0.36.2 && \
    pip3 install idna==3.11 && \
    pip3 install ImageIO==2.37.3 && \
    pip3 install imageio-ffmpeg==0.6.0 && \
    pip3 install importlib_metadata==9.0.0 && \
    pip3 install importlib_resources==6.5.2 && \
    pip3 install ipaddress==1.0.23 && \
    pip3 install ipython==9.11.0 && \
    pip3 install ipython_pygments_lexers==1.1.1 && \
    pip3 install jedi==0.19.2 && \
    pip3 install Jinja2==3.1.6 && \
    pip3 install joblib==1.5.3 && \
    pip3 install julius==0.2.7 && \
    pip3 install kiwisolver==1.5.0 && \
    pip3 install lazy-loader==0.5 && \
    pip3 install librosa==0.11.0 && \
    pip3 install llvmlite==0.46.0 && \
    pip3 install Markdown==3.10.2 && \
    pip3 install markdown-it-py==4.0.0 && \
    pip3 install markdown2==2.5.5 && \
    pip3 install MarkupSafe==3.0.3 && \
    pip3 install matplotlib==3.10.8 && \
    pip3 install matplotlib-inline==0.2.1 && \
    pip3 install mdurl==0.1.2 && \
    pip3 install mmengine==0.10.7 && \
    pip3 install mova==0.1.0 && \
    pip3 install mpmath==1.3.0 && \
    pip3 install msgpack==1.0.8 && \
    pip3 install networkx==3.6.1 && \
    pip3 install ninja==1.13.0 && \
    pip3 install numba==0.64.0 && \
    pip3 install numpy==2.4.3 && \
    pip3 install opencv-python==4.13.0.92 && \
    pip3 install parso==0.8.6 && \
    pip3 install pexpect==4.9.0 && \
    pip3 install pillow==12.1.1 && \
    pip3 install platformdirs==4.9.4 && \
    pip3 install pooch==1.9.0 && \
    pip3 install promise==2.3 && \
    pip3 install prompt_toolkit==3.0.52 && \
    pip3 install protobuf==3.19.6 && \
    pip3 install psutil==7.2.2 && \
    pip3 install ptyprocess==0.7.0 && \
    pip3 install pure_eval==0.2.3 && \
    pip3 install pycparser==3.0 && \
    pip3 install Pygments==2.19.2 && \
    pip3 install PyJWT==2.12.1 && \
    pip3 install pyloudnorm==0.2.0 && \
    pip3 install pyOpenSSL==26.0.0 && \
    pip3 install pyparsing==3.3.2 && \
    pip3 install pystoi==0.4.1 && \
    pip3 install python-dateutil==2.9.0.post0 && \
    pip3 install PyYAML==6.0.3 && \
    pip3 install randomname==0.2.1 && \
    pip3 install regex==2026.2.28 && \
    pip3 install requests==2.32.5 && \
    pip3 install rich==14.3.3 && \
    pip3 install safetensors==0.7.0 && \
    pip3 install schedule==1.2.2 && \
    pip3 install scikit-learn==1.8.0 && \
    pip3 install scipy==1.17.1 && \
    pip3 install sentry-sdk==2.56.0 && \
    pip3 install setproctitle==1.3.7 && \
    pip3 install setuptools==80.10.2 && \
    pip3 install shortuuid==1.0.13 && \
    pip3 install six==1.17.0 && \
    pip3 install smmap==5.0.3 && \
    pip3 install soundfile==0.13.1 && \
    pip3 install soxr==1.0.0 && \
    pip3 install stack-data==0.6.3 && \
    pip3 install sympy==1.14.0 && \
    pip3 install tensorboard==2.20.0 && \
    pip3 install tensorboard-data-server==0.7.2 && \
    pip3 install termcolor==3.3.0 && \
    pip3 install threadpoolctl==3.6.0 && \
    pip3 install tokenizers==0.22.2 && \
    pip3 install tqdm==4.67.3 && \
    pip3 install traitlets==5.14.3 && \
    pip3 install transformers==4.57.6 && \
    pip3 install triton==3.6.0 && \
    pip3 install typing_extensions==4.15.0 && \
    pip3 install urllib3==1.26.20 && \
    pip3 install wcwidth==0.6.0 && \
    pip3 install Werkzeug==3.1.7 && \
    pip3 install wheel==0.46.3 && \
    pip3 install wrapt==2.1.2 && \
    pip3 install yapf==0.43.0 && \
    pip3 install yunchang==0.6.4 && \
    pip3 install zipp==3.23.0


==> arxiv_meow-2/sec/0_abstract.tex <==
\begin{abstract}


Test-Time Tuning (TTT) on pretrained diffusion models has emerged as a powerful paradigm for video editing. However, there exists a foundational mismatch between the distribution-mapping nature of generative models and the single-point optimization of standard TTT. In this paper, we demonstrate that this mismatch triggers \textit{Prior Collapse}, a degenerate state where the model discards the text conditions and spatial latents, collapsing generations to the source video, or entangling the features of distinct regions. To resolve this, we propose \textbf{ElasticTTT}, a novel framework that preserves the prior generative distribution and rescues generative elasticity. Specifically, we propose \textit{Target Distribution Regularization} to prevent sharp memorization minima, \textit{Contrastive CFG} to guide inference away from source biases, and \textit{Asynchronous Noise Schedule} to preserve unedited regions. Extensive evaluations, supported by theoretical analysis, demonstrate that ElasticTTT successfully preserves the generative prior of the base model, achieving state-of-the-art performance on one-shot video editing.


\end{abstract}

==> arxiv_meow-2/sec/1_intro.tex <==
\section{Introduction}

Advancements in denoising diffusion models~\cite{ho2020denoising, song2020score} have enabled significant progress in text-to-video generation~\cite{kong2024hunyuanvideo,wan2025wan,hong2022cogvideo,yang2025cogvideox}. These powerful video generation backbones also open new opportunities for controllable video editing by leveraging learned generative priors~\cite{DBLP:journals/corr/abs-2503-11412,mou2024revideo,huang2025dive}. However, user-provided source videos may fall outside the fixed training distribution of off-the-shelf models~\cite{yu2025veggie,bai2025ditto, zi2025se, wu2025insvie, he2025openve,li2025qffusion, bian2025videopainteranylengthvideoinpainting,zhang2025voicebridge}, particularly given the rapid emergence of new concepts across the internet, resulting in degraded editing performance. Recently, another line of research has explored Test-Time Tuning (TTT)~\cite{sun2020test, wang2020tent,wang2025low,wu2023tune, huang2025dive, Harsha_2024_CVPR, wang2025t3v2v}, which aims to adapt the weights of off-the-shelf models to the domain of user-provided source videos.

% , allowing more consistent and faithful video editing performance without any large scale training cost.

Compared with video editing approaches that perform inference directly with pre-trained models, TTT is particularly well suited to challenging scenarios where the source video exhibits a large domain gap from the pretraining distribution. This is because TTT explicitly adapts the model to the specific content and dynamics of each source video, thereby improving the preservation of its appearance, structure, and motion. Besides serving as a practical paradigm for video editing, TTT-based methods also function an effective data engine for synthesizing paired editing data to train large-scale feed-forward video editing models~\cite{wu2025insvie,zi2026senorita}.


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/qualitative_comparison.jpg}
    \vspace{-8mm}
    \caption{Demonstration of ElasticTTT and the baseline TTT method on four different editing tasks. ElasticTTT obtains high quality editing results among all tasks, whereas the baseline method exhibits clear Conditioning Collapse and Spatial Entanglement.}
    \label{fig:demo}
    \vspace{-3mm}
\end{figure}


Although TTT provides a natural mechanism for personalized user experiences~\cite{ruiz2023dreambooth, bi2025customttt, gal2022image, kumari2023multi,wu2026pipbench}, it introduces an inherent tension with the diffusion process: TTT intentionally encourages instance-specific overfitting, while diffusion processes are inherently stochastic and intended to preserve distributional diversity. Notably, optimizing a highly parameterized diffusion model exclusively on this zero-variance singularity can easily lead to a failure mode that we term \emph{prior collapse}. As illustrated in~\cref{fig:demo}, prior collapse manifests itself in two complementary failure phenomena. \emph{Conditioning Collapse} arises when the conditional guidance becomes anchored to the source-conditioned dynamics during tuning, preventing effective semantic control and causing the model to disregard the target editing instruction. \emph{Spatial Entanglement} arises when spatial representations become globally coupled during denoising, preventing localized control and causing unintended modifications outside the target region.



To circumvent these challenges, previous methods have proposed a spectrum of interventions. To mitigate Conditioning Collapse, prior works often rely on low-rank adaptation (LoRA)~\cite{gao2025lora}, prior-preservation losses~\cite{ruiz2023dreambooth}, self-supervised objectives~\cite{wang2025low}, or the isolated optimization of text and null-text embeddings~\cite{gal2022image, mokady2023null}. To resolve Spatial Entanglement, methods typically resort to invasive attention map modifications~\cite{kwon2024unified,zuo2025cut}, masked optimization phases~\cite{gao2025lora}, or the injection of external control signals like depth and optical flow~\cite{wang2025t3v2v}.
However, these approaches are fundamentally sub-optimal, their complexity determines that they heavily rely on delicate architectural tuning, require auxiliary datasets, or remain dangerously sensitive to hyperparameter choices.


More importantly, while Test-Time Tuning (TTT) has shown immense promise in image editing by fine-tuning models directly on the source image, adapting TTT to video is remarkably scarce and fraught with difficulty. Video Diffusion Transformers~\cite{wan2025wan,peebles2023scalable} possess highly complicated spatial-temporal priors, and naively transferring image-based TTT optimization techniques to video models severely accelerates Prior Collapse. The network quickly overfits to the deterministic motion and appearance of the source video, losing its generative elasticity required for precise, accurate editing.

\begin{comment}
    
While recent advancements have explored fine-grained video editing, balancing editing flexibility with structural loyalty remains a persistent challenge. Many approaches rely on delicate architectural interventions—such as manual attention control—which struggle to generalize from traditional U-Nets to modern Diffusion Transformers (DiTs). Others attempt to mathematically guide the diffusion process but fail to consistently balance flexibility and fidelity due to rigid hyperparameters applied uniformly across varying tasks. Alternatively, injecting auxiliary information like depth or segmentation masks often requires cumbersome manual user inputs or extensive, resource-heavy fine-tuning. More importantly, while Test-Time Tuning (TTT) has shown immense promise in image editing by fine-tuning models directly on the source image, adapting TTT to video is remarkably scarce and fraught with difficulty. Video diffusion models possess highly complex spatial-temporal priors; existing image-based TTT methods cannot simply be adapted to video without the model rapidly overfitting and losing its generative capabilities.

\end{comment}
% \C{I think The following paragraph could be deleted completely. The previous para did its functions}
% \ML{this paragraph need rewrite. We need a high level sentence on how those works solve the above issues, and why we they didn't solve those issues as they intended to}
% Previous methods leverage multiple techniques and delicate structure to achieve fine-grained video editing while maintaining the basic motion in the reference video. Some works~\cite{yang2025videograin,DBLP:conf/icassp/WangZ0CG025}try to manually control attention weight but face problems when changing U-net to DIT. Other works~\cite{kim2026flowalign,kulikov2025flowedit} explore a mathematical way to guide the diffusion process but meet problems while balancing editing flexibility and motion loyalty due to the fixed hyperparameter for all images and editing tasks. The others~\cite{chen2025perception,bian2025videopainter,burgert2025motionv2v}try to inject more information such as depth or segmentation masks into the diffusion models but require large finetuning process and additional user input. \ML{be more intutive on why previous method did not address this issues. another issues is that it not looks alike a lot of videoTTT, but in fact not that many (since we don't have much TTT to compare based on our discussion). we need to make it clear that some methods are not on video and can not be adapted ti video}

% \C{Question / Concern: Is this weighting correct? I thought in more papers that the descriptions of methods, rather than the problem settings, should take the most spaces. It seems common practice will assign one paragraph each for the 3 mechanisms. Are we doing this right?}
% \ML{this para is too dense, the intro of methods should be high-level and intutive. let me try something}
\begin{comment}
To resolve this fundamental optimization–sampling tension, we propose \textbf{ElasticTTT}, a principled framework that reconciles the competing objectives of source preservation and target editing across the entire diffusion-based TTT pipeline, spanning optimization, guidance, and sampling. At the optimization stage, we introduce \emph{Target Distribution Regularization}, which preserves the model’s elastic denoising behavior by softly relaxing the rigid optimization target through injecting controlled stochasticity. For conditioning guidance, we introduce \emph{Contrastive Classifier-Free Guidance}, which decouples embedded source concepts by explicitly opposing the target condition to the source. At the sampling stage, we introduce \emph{Asynchronous Noise Scheduling}, which dynamically assigns independent diffusion trajectories to edited and preserved regions to mitigate Spatial Entanglement. 
\end{comment}

To resolve this fundamental optimization–sampling tension, we propose \textbf{ElasticTTT}, a principled framework designed to rescue generative elasticity and explicitly cure the symptoms of Prior Collapse. Rather than treating these failures as isolated artifacts, ElasticTTT intervenes across the entire generative pipeline: First, to prevent Conditioning Collapse during optimization, we introduce \emph{Target Distribution Regularization}. By softly relaxing the rigid, single-point target with controlled stochasticity, we physically prevent the model from memorizing the source video, preserving its elastic denoising priors. However, as the tuned weights still exhibit a residual shift toward the source concept, we subsequently apply \emph{Contrastive Classifier-Free Guidance} during inference to forcefully steer the trajectory toward the target condition. Finally, to resolve Spatial Entanglement, we introduce an Asynchronous Noise Schedule in the sampling process, which dynamically assign independent diffusion trajectories to the edited and anchored regions, clarifying latent representations and granting the model the localized freedom to render new concepts while safely preserving the unedited surroundings.
% \ML{please check, still sound  abit piling things up}

To validate the effectiveness of our framework, we conduct extensive experiments across a diverse range of editing tasks. Our results demonstrate that ElasticTTT successfully resolves the prior collapse issue, exhibiting robust generative elasticity, precise instruction adherence, and high-fidelity preservation of the source video. In both quantitative and qualitative evaluations, ElasticTTT consistently outperforms competitive baselines—spanning inference-only, test-time-tuning, and training-based approaches—ultimately achieving state-of-the-art performance in video editing.




% To resolve this fundamental optimization–sampling tension, we propose \textbf{ElasticTTT}, a principled framework that reconciles the competing objectives of source preservation and target editing across the entire diffusion-based TTT pipeline, spanning optimization, guidance, and sampling. 

% First, to prevent the model from bypassing the conditional information and collapsing into a deterministic reconstruction of the source video, we introduce \textbf{Target Distribution Regularization} (TDR). By softening the rigid optimization target into a continuous local distribution through injecting geometry-aware noise, TDR prevents deterministic memorization and retains the model's elastic denoising properties.

% Second, to further cancel out the distribution shift toward the source video, we propose \textbf{Contrastive Classifier-Free Guidance (Contrastive CFG)}. This mechanism contrasts the target condition against the source and guide the generation process along this direction, explicitly decoupling the embedded source concepts. 
% Finally, we address Spatial Entanglement during inference with \textbf{Asynchronous Noise Scheduling (Async-NS)}. Powered by a fully automated, zero-shot vision-language segmentation pipeline, Async-NS dynamically assigns independent flow trajectories to edited and preserved regions. This mechanism grants the model the semantic freedom to aggressively overwrite target concepts and sufficient information to reconstruct unedited regions, and clarifying the latent representations through distinct time embeddings among regions.

\begin{comment}
To this end, we propose \emph{ElasticTTT} that address the prior collapse challegen in a principled view: collapse occurs when tuning destroys distributional flexibility, semantic controllability, and spatial locality. Accordingly, we restore these three properties in a coordinated manner. First, \ML{this is the first time TDR show up, you need to explain, and I don't think we new abbrivation here, only in method and epxeriements when same words brought up frequently}TDR softens the target training distribution during tuning, preventing the model from collapsing into deterministic reconstruction of the source video. Second, Contrastive Classifier-Free Guidance introduces contrast against the source condition, explicitly pushing generation away from source-specific semantics and toward the target editing instruction. Third, Async-NS separates the denoising dynamics of edited and preserved regions, reducing spatial interference and preventing unintended modifications. \ML{please check... really not sure. too much details for me to understand fully}

Consider the examples in Fig.~\ref{fig:demo}. \ML{combine example and explain the two issues}
\end{comment}



% Recent advancement in video generation models~\cite{kong2024hunyuanvideo}~\cite{hong2022cogvideo}~\cite{wan2025wan}~\cite{yang2025cogvideox},especially Text-to-video models,have achieved huge success and are capable of generating vivid videos with natural language instructions. These highly effective pretrained base models enable many downstream applications such as video editing. In a practical application, enabling users to modify reference videos according to their own preferences is a meaningful task. Users can express their creative ideas only in natural language, avoiding complicated and annoying editing tools. 

% \C{Para1: start with T2V or video editing? video editing -> TTT or general TTT algorithms?}

% However, we noticed a foundational mismatch between the standard TTT paradigm and core generative framework of diffusion models. Generative models are trained to map a noise prior to a diverse, continuous data distribution, whereas in single-video TTT, the training data distribution violently collapses to a single sample. Optimizing a highly parameterized diffusion model exclusively on this zero-variance singularity leads to an effect we formally identify as \textbf{prior collapse}, causing existing TTT systems to be vulnerable in three ways:

%Some other one-shot tuning methods are usually extremely sensitive to hyperparameter settings and require hundreds of steps of finetuning.

\begin{comment}
  To address these issues, we introduce a novel universal test-time-tuning(TTT) pipeline. The main advantages of our pipeline can be summarized into four main parts:

\begin{itemize}
\item Zero additional parameters and no need for extensive fine-tuning.

\item Able to leverage any Text-to-Video models no mater the basic structure is 2D-Unet,3D-Unet or DIT 

\item Nearly all editing tasks are available in the same pipeline with only natural languages instructions(object-editing, style editing, background editing, class editing and etc)

\item Hyperparameter Robustness
\end{itemize}

To achieve these, our key insights are 1) Async-NS in different part of the video
2) 
3) Perform additional classification paranoia during reasoning may also help improve the quality of the edited video. 

Our key contribution can be summarized as follows:


\begin{itemize}

  \item To the best of our knowledge, this is the first attempt at Cross-Architecture universal Test-Time-Tuning (TTT) Pipeline

  \item We propose TTT, a novel Test-Time-Tuning  pipeline that utilizing Async-NS By mapping the distribution, VidTTT achieves robust performance on hyperparameter and rapid adaptation with fewer TTT steps.

   \item Our method not only achieves state-of-art performance with 70 tuning steps but also yields impressive results with as few as 20 TTT iterations.
\end{itemize}
  
\end{comment}


==> arxiv_meow-2/sec/2_related.tex <==
\section{Related work}
\subsection{Test-Time Tuning of Diffusion Models}

Test-Time Tuning (TTT)~\cite{sun2020test, wang2020tent} updates a pre-trained diffusion model at inference time for tasks like customized and personalized generation~\cite{ruiz2023dreambooth, kumari2023multi, gal2022image, bi2025customttt}, stylized generation~\cite{zhang2023inversion, chung2024style, sohn2023styledrop, wang2023stylediffusion}, and test-time scaling~\cite{ma2025inference}.  For generative editing, TTT establishes a high-fidelity anchor by reconstructing a specific reference video~\cite{wu2023tune} for subsequent modifications, but optimizing the model on a single reference naively often degenerates performance~\cite{ruiz2023dreambooth}. Previous works attempt to mitigate this issue via low-rank adaptation~\cite{gao2025lora, gal2022image}, additional prior-preserving losses~\cite{ruiz2023dreambooth}, only optimizing text embedding~\cite{gal2022image} or null-text embeddings~\cite{mokady2023null}, or introducing self-supervised signals~\cite{wang2025low}. However, these interventions do not fully resolve the issue, especially on highly parameterized text-to-video models~\cite{wan2025wan}, often resulting in a zero-sum compromise between following novel editing instructions and preserving details of the source video.

\subsection{Video Editing}
Video editing requires seamlessly integrating new semantic concepts or modifying existing features while preserving the source video's unedited structures. Existing methods generally fall into three paradigms. \textit{Training-based methods}~\cite{yu2025veggie,bian2025videopainteranylengthvideoinpainting,DBLP:journals/corr/abs-2503-11412,li2025qffusion, wu2025insvie, he2025openve, bai2025ditto, zi2025se} fine-tune video generation models on paired datasets, but suffer from severe data scarcity and limited generalization on new concepts, and heavy computational resources needed for training. \textit{Training-free methods}~\cite{kulikov2025flowedit,cohen2024slicedit,DBLP:journals/corr/abs-2403-16111, ku2024anyvv, geyer2024tokenflow, jeong2024groundavideo, bai2025uniedit,liu2025stablev2v} bypass data requirements by leveraging pre-trained priors via inverse diffusion methods~\cite{song2020denoising, meng2021sdedit}, often including manipulating attention maps~\cite{meral2024motionflow,liu2025stablev2v,kwon2024unified} or utilizing pretrained image editing models~\cite{DBLP:journals/corr/abs-2405-16537,gao2025lora,ku2024anyvv,liu2025stablev2v}, but inherently struggle to balance semantic alignment and reference preservation due to fixed model parameters and sampling trajectory length. \textit{Test-Time Tuning (TTT) methods}~\cite{wu2023tune,huang2025dive,Harsha_2024_CVPR,liu2024video} bridge this gap by tuning the base model directly on the source video, improving source reconstruction without involving external datasets. However, adopting TTT for video editing directly encounters the prior collapse issue, to which we offer a systematic solution in our work. More details of the related works are shown in Supplementary.

\begin{comment}
Previous methods 

The previous methods can be roughly divided into four main approaches. First,some methods utilized a two-stage approach(image editing + image guide video generation)~\cite{gao2025lora,DBLP:journals/corr/abs-2405-16537}.Although these methods yield fine-grained video generation results, they face difficulties in handling significant motion changes and exhibit an over-reliance on image editing models. 
The second kind of methods uses mathematical techniques~\cite{kim2026flowalign,kulikov2025flowedit}to guide the diffusion process. Although these training-free methods are highly efficient, they often suffer from limited editing flexibility.
The third comprises attention-driven methods~\cite{DBLP:journals/corr/abs-2412-05275,ku2024anyvv,liu2025stablev2v}, which achieve spatial decoupling and controllable editing by manipulating self- and cross-attention maps. However, these approaches face significant challenges when adapted to DiT~\cite{peebles2023scalable} architectures.
The fourth category of methods relies on fine-tuning models in domain-specific video editing datasets.~\cite{bai2025ditto,yu2025veggie,bian2025videopainteranylengthvideoinpainting}. Many previous works add additional tokens or structures to help the base model fit the needs of different video editing tasks. However, such methods often require computationally expensive fine-tuning and tend to introduce dataset-specific biases. For example, approaches that rely on datasets from simulated environments often suffer from texture degradation and game-like artifacts in their outputs. In contrast, our proposed method achieves state-of-the-art performance while ensuring a manageable computational overhead.
\end{comment}
\begin{comment}
\subsection{Controllable Video generation}
Developing controllable video generation techniques is crucial for practical applications. The primary dimensions of controllable generation include camera, motion, and semantic control. For instance, Any-Traj~\cite{wang2025ati} utilizes user-specified trajectories to formulate spatial Gaussian distributions as guidance signals for diffusion models, though it requires extensive fine-tuning. For semantic control, Video-as-Prompt~\cite{bian2026videoasprompt} duplicates the pre-trained model into a trainable 'expert' to process reference videos, interacting with the frozen base model via in-context full attention. It also introduces a temporal RoPE bias to prevent spurious spatiotemporal references. To manage computational overhead, OpenVE-3M~\cite{he2025openve} employs a Mixture-of-Experts (MoE) connector and an MLLM to efficiently process fine-grained instructions. Finally, for camera control, RecamMaster~\cite{bai2025recammaster} concatenates the reference video with initialized noise along the temporal dimension, achieving highly effective and decoupled camera manipulation
\end{comment}
\begin{comment}
Creating controllable videos is a meaningful study for practical applications.The main categories of controllable video generation are camera control, motion control and semantic control. Any-Traj~\cite{wang2025ati} utilizes the user-given trajectory to form a spatial Gaussian distribution as a guidance signal for diffusion models but requires massive finetuning. Video-as-Prompt~\cite{bian2026videoasprompt} deal with video sementic control by copying the pretrained model as an trainable "expert-model" to process reference video and interact with the frozen pretrained model through in-context full attention. A temporal RoPE bias is also used to avoid unexisting temporal spacial reference. OpenVE-3M~\cite{he2025openve} utilizes MoE connector and MLLM to gain fine-grained instructions while mitigating huge computation cost. RecamMaster~\cite{bai2025recammaster} concat the reference video to the initialized noise in time dimension,achieving fantastic and decoupled camera control. 
\end{comment}



\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{fig/pipeline_overview.jpg}
    \vspace{-9mm}
    \caption{\textbf{The overall pipeline of ElasticTTT}. To resolve Conditioning Collapse, we soften the optimization target via TDR during training, and repel the sampling process from the source distribution via Contrastive CFG during sampling. To mitigate Spatial Entanglement, we perform Asynchronous Noise Scheduling to establish independent integration trajectories for distinct regions.}
    \label{fig:pipeline}
    \vspace{-3mm}
\end{figure}


==> arxiv_meow-2/sec/3_method.tex <==
\section{Method}

\label{sec:overview}

Given a source video $V_{\text{src}}$ and its corresponding descriptive text prompt $C_{\text{src}}$, the goal of video editing is to generate a target video $V_{\text{trg}}$ that aligns with a user-provided target prompt $C_{\text{trg}}$ while preserving the fundamental structural and temporal dynamics of $V_{\text{src}}$. Standard video editing models sample from a fixed conditional distribution 
$p_{\theta}(V_{\text{trg}}\mid V_{\text{src}}, C_{\text{trg}})$ with frozen parameters $\theta$, 
whereas test-time tuning approaches first adapt the model parameters on the source input via 
$\theta' = \mathcal{A}(\theta; V_{\text{src}}, C_{\text{src}})$, 
and then sample from the instance-adapted distribution 
$p_{\theta'}(V_{\text{trg}} \mid V_{\text{src}}, C_{\text{trg}})$, 
allowing stronger identity preservation and scene-specific consistency under the desired editing prompt.

Concretely, in the first stage, the model operates in a latent space and is optimized to reconstruct the source video latent $x_0$ by minimizing the MSE loss between the predicted velocity $v_\theta$ and the target conditional vector field $u_t$ given the noised latent $x_t$ at timestep $t$:
\begin{align}
    \mathcal{L}_{\text{TTT}} = \mathbb{E}_{t, x_t} \left[ \lVert v_\theta(x_t, t, C_{\text{src}}) - u_t(x_t \mid x_0) \rVert^2 \right]
\end{align}
Once the model is fine-tuned, inference is performed starting from a noisy latent, acquired by DDIM inversion~\cite{song2020denoising}, utilizing the target prompt $C_{\text{trg}}$ to guide the generation of $V_{\text{trg}}$.



\subsection{The Optimization–Sampling Tension}
While standard TTT captures the spatial-temporal features of the reference video, it introduces a fundamental mismatch with the generative nature of diffusion models.
Diffusion models learn mappings between data distributions and rely on diverse samples to preserve generative flexibility. In TTT, however, the distribution of training data collapses to a single instance, effectively degenerating into a Dirac delta distribution, i.e., $p(x)=\delta(x-x_0)$. 

Optimizing a highly parameterized diffusion model on such a single-point distribution can easily lead to a failure mode that we term \textbf{\textit{prior collapse}}: The model overfits to high-frequency pixel-level details of the source video, prioritizing exact reconstruction over generalizable condition-aware denoising. We conducted an illustrative experiment to examine this phenomenon, as shown in~\cref{fig:toy}: The base diffusion model is trained on a distribution with 25 classes (A), and TTT is performed on one sample of the center class. When we conduct inference with other class conditions, the model simply bypasses the conditions and generates a chaotic cluster around the memorized target distribution (B).

Formally, in video diffusion models, the network predicts the velocity field $v_\theta(x_t, t, C_\text{src})$ based on the noisy latent $x_t$ and the text condition $C_\text{src}$. Although the large pretrained model does not fully collapse the prior distribution, it still progressively learns to bypass meaningful variations in $x_t$ and $C_\text{src}$, instead hard-coding the high-frequency details of the source video into its parameters, degrading editing performance across two modalities:


\begin{itemize}
    \item \textbf{Conditioning Collapse} By repeatedly updating on a static text prompt $C_\text{src}$, the model gradually weakens the text condition pathways. This causes the model to ignore the target prompt $C_\text{trg}$ during inference, losing its semantic elasticity, anchoring to the source concept rather than following new textual guidance (\cref{fig:demo} first row).
    \item \textbf{Spatial Entanglement} By increasingly bypassing the noisy input $x_t$ to memorize the global target, the model degrades its ability to extract semantically meaningful spatial representations from $x_t$. Consequently, distinct semantic objects lose their boundaries, causing severe visual corruption and entanglement when attempting to edit specific regions (\cref{fig:demo} second row).
\end{itemize}
\begin{figure}[tbp]
    \centering
    \vspace{-3mm}
    \includegraphics[width=1\linewidth]{fig/toy_experiment.jpg}
    \vspace{-8mm}
    \caption{A 2D toy experiment, illustrating the effect of TDR and Contrastive CFG. In standard TTT, the generated distribution of the base model (A) collapses around the optimization target (B), and dispersing to chaos when CFG is applied (C, D). With TDR, the generated distribution remains its original structure (F), and Contrastive CFG further cancels out the introduced distribution shift (G, H).}
    \label{fig:toy}
    \vspace{-5mm}
\end{figure}
Importantly, prior collapse is not equivalent to overfitting: TTT intentionally encourages controlled overfitting to capture source characteristics, while prior collapse represents a degenerate regime in which generative behavior collapses and editing controllability is lost. 

To resolve this foundational mismatch, we propose \textbf{ElasticTTT}, a novel pipeline that preserves the generative prior. We mitigate Conditioning Collapse during training by softening the optimization target into a continuous local distribution~\cref{subsec:TDR}, and resolve the remaining conditioning bias induced through repelling the generation from the source condition through a contrastive classifier-free-guidance~\cref{subsec:contrastivecfg}. We resolve Spatial Entanglement during inference by dynamically processing different regions with asynchronous noise levels~\cref{subsec:asyncns}. The following sections detail the formulations of these three methods.

\begin{comment}
In practice, three fundamental challenges arise. 


Firstly, $V^*$ must maintain the complex motion dynamics of $V$, particularly when handling rapid or intricate movements. Secondly, video editing models typically exhibit overfitting to simple prompts, constraining their capacity to generalize across diverse textual descriptions. This overfitting phenomenon, commonly observed in both text-to-image and text-to-video models. Thirdly, due to the lack of huge datasets,all existing one-shot-tuning methods are quite sensitive to hyperparameter and the detailed reasons will be illustrated in Section3.4. 

 Our approach incorporates three complementary tasks: (i) employing masked auto-encoding in detected motion regions to guide the reconstruction of video latent representations, thereby enforcing motion consistency; and (ii) utilizing a synchronous noise scheduling to balance motion loyalty and semantic alignment
(iii) utilizing a distribution mapping method to achieve high robust in hyperparameter and improving editing flexibility.  By simultaneously enhancing temporal consistency and semantic fidelity, our method produces videos with smooth motion patterns and precise edits.
\end{comment}



\begin{comment}
    
\subsection{Spatial-temporal representation learning}
\label{sec:spatiotemporal}


To effectively capture and preserve motion dynamics in videos, we introduce an adaptive spatio-temporal representation learning approach that focuses on key motion regions. Our method begins with object detection to localize moving entities, followed by optical flow analysis to identify significant motion areas.

Specifically, we apply YOLOv8~\cite{redmon2016lookonceunifiedrealtime} to perform object detection on each frame $f_t$ of the video, producing a bounding box $B_t = (x_t, y_t, w_t, h_t)$. Given a video tensor $v \in \mathbb{R}^{T \times C \times H \times W}$, we partition each frame into patches of size $p_h \times p_w$. The total number of patches per frame is:
\begin{equation}
N_p = (H/p_h) \times (W/p_w).
\end{equation}
Within the bounding box $B_t$, the number of patches covering the object is:
\begin{equation}
N_{B_t} = (h_t/p_h) \times (w_t/p_w).
\end{equation}
We define mask ratios $r_f$ and $r_b$ for the object and background regions, respectively. The number of patches to be masked is:
\begin{equation}
M_f = r_f \cdot N_{B_t}, \quad M_b = r_b \cdot (N_p - N_{B_t}).
\end{equation}

Subsequently, we utilize GMFlow~\cite{xu2022gmflow} to compute the optical flow $F_t$ between consecutive frames and derive a motion intensity $m_t(i)$ for each patch. Patches within $B_t$ are ranked by their motion intensity, with the top $M_f$ patches selected for masking, while $M_b$ background patches are randomly masked. The resulting mask $M_t$ is applied to the clear latent representation $z_t$ from the VAE encoder: $\tilde{z}_t = M_t \odot z_t$, where $\odot$ denotes element-wise multiplication. The video reconstruction loss is:
\begin{equation}
\mathcal{L}_{mse} = \frac{1}{N} \sum_{i=1}^{N} \lVert M_{pred}(N(\tilde{z}_t(i))) - z_t(i) \rVert_2^2.
\end{equation}

where N(*) represents the noise adding formula in the inversion process and $M_{\text{pre}} $ represents the single-step denoising prediction in diffusion models.

This targeted approach enables the model to focus on the most challenging dynamic elements of the video. By strengthening the reconstruction of the most dynamic area, the diffusion model are able to learn the motion trajectory in the reference video and improve the motion loyalty in the edited video.

%\subsection{Semantic Contractive Learning}
%\label{sec:semantic}

%To address prompt overfitting, we develop a semantic representation space exploration framework that enhances model generalization through systematic prompt perturbation. Given an original editing prompt $T$, we generate a set of augmented prompts $\{T_a^i\}_{i=1}^n$ that preserve the semantic content while exploring different regions of the text representation space.

%Our augmentation strategy employs three primary techniques: back-translation, synonym replacement, and syntactic reformation. These techniques produce semantically equivalent prompts that differ in expression, enabling the model to learn more robust mappings in the text representation space.
%Our further study illustrates that only using GPT-2 to produce augmented prompts can achieve similar results too.


%Subsequently, we implement a contractive learning task. We apply a random masking strategy to the augmented prompts, replacing selected tokens with \texttt{[MASK]} tokens to generate masked prompts $T_m$. These masked prompts are processed through the T5 encoder and a pretrained linear network in Wan model to produce hidden representations $Z_m$. The clean augmented prompts and the original prompts are also proposed through the above structure to generate the hidden representation $Z_a$ and $Z_o$ respectively. 

%Moreover, we also proposed masked and non-masked reference video through VAE and another pretrained MLP in Wan to generate video's hidden representation $H_m$ and $H_v$ respectively.

%Because the pretrained two linear layers in Wan model aim to project the video and the text into the same semantic space, we are able to compare the similarity between text and video latent.

%We define the similarity between video and text latent as following:

%\[
%\mathbf{z}_i = \frac{\mathbf{Z}_i}{\lVert \mathbf{Z}_i \rVert}, 
%\mathbf{h}_j = \frac{\mathbf{H}_j}{\lVert \mathbf{H}_j \rVert}, 
%\quad
%s_{ij} = \mathbf{z}_i^\top \mathbf{h}_j
%\]

%where $z_i$ is the normalized feature of $Z_i$ and $h_i$ is the normalized feature of $H_i$. To conduct the contrastive learning, we define the positive sample set as follows:

%\[
%P=\{(Z_m,H_m),(Z_v,H_v)\},\quad
%\]

%By strengthening the similarity between $z_m$ and $h_m$, the model is able to capture and predict the semantic information only based on part of the text and video, preventing the overfitting on only a few words or part of the reference video. However,only adding this noise is not enough due to the limited test-time-tuning steps and only a single reference data. The model is easy to capture some strange and odd correlation between video and text. Therefore, strengthening the similarity between the non-masked hidden representation is also quite necessary. This similarity guidance provides a baseline for model to further explore and predict without going astray. We propose our contractive loss as follows:
%\[
%\mathcal{Q}_{\text{ij}}
%=\exp(s_{ij}/\tau)
%\]
%\[
%\mathcal{L}_{\text{con}}
%=
%\frac{1}{|P|}
%\sum_{(Z_i,h_j)\in P}
%-\log
%\frac{{Q}_{\text{ij}}}
%{{Q}_{\text{ij}}+\sum_{(Z_a,h_b)\notin P}{Q}_{\text{ab}}}
%\]
%\end{equation}
%This self-supervised approach compels the model to learn more robust text representations capable of handling various textual variations, thereby mitigating prompt overfitting.

%Overall,our total loss is defined as follows:
%\[
%\mathcal{L}_{\text{con}}
%= {L}_{\text{noise}}+\lambda_{\text{mse}}\){L}_{\text{mse}}+\lambda_{\text{com}}\){L}_{\text{com}}
%\]
%where \lambda_{\text{mse}}\)and \lambda_{\text{com}}\) are two hyper parameters.
\end{comment}


\begin{comment}
A fundamental challenge of Test-Time-Tuning (TTT) in video generation is the extreme scarcity of training data. During TTT, the empirical data distribution consists of a single reference video, forming a Dirac delta distribution $p_{data}(x) = \delta(x - x_0)$. 
When a highly parameterized diffusion model is optimized toward this single point, it rapidly collapses into a state of exactly memorizing the source data, instead of completing the regular denoising mission. This phenomena, which we call the "prior collapse", commonly happen after 100 training steps, where the model generates only the source video regardless of the editing instructions. The optimization trajectory becomes entangled with the specific details of the source video, destroying the network's semantic generation ability from new text conditions.

the model is optimized on a single reference video, forming a Dirac delta distribution $p_{data}(x) = \delta(x - x_0)$. Optimizing a highly parameterized network on this single point encourages the model to learn a shortcut by directly memorizing $x_0$ inside its parameters, instead of learning useful representations of the latent $x_t$ and condition $C_\text{src}$ for denoising purpose. This phenomena, which we call the \textit{prior collapse}, collapses the learned representations and destroys the general denoising capability of the pretrained video model.
\end{comment}

\subsection{Target Distribution Regularization: Escaping the Dirac Singularity}
\label{subsec:TDR}
The root cause of Prior Collapse of the standard TTT lies in the rigid and deterministic nature of the Dirac delta distribution $p_{data}(x) = \delta(x - x_0)$ of the target data. To prevent the generative prior from collapsing into this sharp singularity, we introduce \textit{Target Distribution Regularization} (TDR).

The core insight of TDR is to inject controlled stochasticity \textit{strictly} into the optimization target, while keeping the input trajectory completely clean. Specifically, given a clean source video $x_0$ and a standard Gaussian noise sample $x_1 \sim \mathcal{N}(0, I)$, we construct the intermediate noisy latent $x_t$ exactly as in standard flow matching $x_t = tx_1 + (1-t)x_0$. 
% However, when computing the target velocity that the network must predict, we construct a perturbed target $\tilde{x}_0$ instead:
However, when computing the target velocity for supervision, we replace the deterministic target $x_0$ with a perturbed version $\tilde{x}_0$: 
\begin{align} \tilde{x}_0 = x_0 + \epsilon_\text{reg}, \quad \epsilon_\text{reg} \sim \mathcal{N}(0, \sigma_\text{reg}^2 I) \end{align}
We then have the following updated optimization target $u_t(x_t|\tilde{x}_0) =  x_1 - \tilde{x}_0$. Note that the model input $x_t$ is interpolated using the original, unperturbed $x_0$ and is completely independent of $\epsilon_\text{reg}$.

Crucially, this stochastic injection does not alter the fundamental optimization objective of the model. In the original flow-matching framework~\cite{lipman2023flow}, the network is trained to predict the conditional expectation of the velocity field:
\begin{align} v^*(x_t, t) = \underset{v}{\arg\min} \, \mathbb{E}_{t, x_0, x_1} \left[ \| v(x_t, t) - u_t(x_t \mid x_0) \|^2 \right] = \mathbb{E}_{x_0 \mid x_t} \left[ u_t(x_t \mid x_0) \right] \end{align}
Because standard flow matching paths construct the velocity field to be linear with respect to the target data (\ie, $u_t(x_t|\tilde{x}_0) = x_1 - \tilde{x}_0 = x_1 - x_0 -\epsilon_\text{reg} - x_t = u_t(x_t|x_0)-\epsilon_\text{reg}$), training the network $v_\theta$ to predict this perturbed velocity field causes the new optimal vector field $\tilde{v}^*(x_t, t)$ to evaluate to:
\begin{align}
\tilde{v}^*(x_t, t) &= \mathbb{E}_{x_0, \epsilon_\text{reg} \mid x_t} \left[ u_t(x_t \mid \tilde{x}_0) \right] = \mathbb{E}_{x_0, \epsilon_\text{reg} \mid x_t} \left[ u_t(x_t \mid x_0) - \epsilon_\text{reg} \right]\\
&= \mathbb{E}_{x_0 \mid x_t} \left[ u_t(x_t \mid x_0) \right] - \mathbb{E}_{\epsilon_\text{reg}} \left[ \epsilon_\text{reg} \right] = v^*(x_t, t)
\end{align}
The injected noise $\epsilon_\text{reg}$ is sampled independently with zero mean, ensuring that the perturbation remains unbiased in expectation. Therefore, the global minimum of our regularized objective remains perfectly aligned with the original video's true vector field.

As shown in the toy experiment in~\cref{fig:toy}, instead of generating a collapsed distribution (B), the generation of the TDR model preserves the structures of the prior distributions (F), highlighting the significance of the introduced stochasticity.
Although the expected target remains identical, the variance $\sigma_\text{reg}^2$ fundamentally alters the optimization dynamics. By replacing the strict Dirac delta point with a continuous local Gaussian manifold, we introduce a geometry-aware variance penalty into the loss landscape. The model thus no longer minimizes the loss by lazily memorizing an infinitely sharp, rigid spatial mapping to $x_0$. Instead, it learns to retain its elastic properties as a denoising model and seeks a broader, generalized minimum. Consequently, the model robustly follows target text prompts even after extensive fine-tuning steps, dramatically increasing editing flexibility and stabilizing the TTT process. A more mathematical explanation is shown in Supplementary~\cref{app:math}.

\begin{comment}

In the experiment,we observed that the existing Test-time-tuning networks are all extremely sensitive to the hyperparameter,especially test-time-tuning steps and the noise schedule of the initial noise. Two extreme phenomena alternately appear when changing the hyperparameter slightly and the quality of the final results experience a stepwise change rather than continuous change. 

We analyze this causes of this phenomenon and propose the following hypothesis due to our experiment and previous theories.

\textbf{Hypothesis 1:}

In the diffusion process,due to the large data used in the training process, these pretrained models have the ability to suppress minor errors$(\epsilon)$ even after hundreds of steps of Test-time-tuning. However,when the error surpass a threshold $(l)$,the diffusion models tend to magnify errors instead of reducing them. Mathematically,this hypothesis can be describe as:

\[
{X}_{\text{t1}}
={X}_{{t2}}-{V}_{\text{}}({X}_{\text{t2}},t2,{C})dt
\]
\[
{Y}_{\text{t1}}={Y}_{\text{t2}}-{V}_{\text{}}({Y}_{\text{t2}},t2,{C}_{\text{}})dt
\]
\[
|X_{t1}-Y_{t1}|<|X_{t2}-Y_{t2}|(if (X_{t2}-Y_{t2})<l)
\]
\[
|Y_{t2}-X_{t2}+{V}_{\text{}}({X}_{\text{t2}},t2,{C})dt-{V}_{\text{}}({Y}_{\text{t2}},t2,{C})dt|<|Y_{t2}-X_{t2}|
\]
where ${C}_{\text{}}$ is the user given prompt.${X}_{\text{t1}}$ and ${X}_{\text{t2}}$ are two noisy latent in the diffusion process$(0<t1<t2<1)$. $V(*)$ is the pretrained velocity prediction network in flow-matching.


\textbf{Hypothesis 2:}


The previous work Flow-align illustrates a finding that the distribution of the edited video remains proximal to that of the source video. We cite this conclusion without further proof.

\textbf{Hypothesis 3:}

When a video is at a low noise level, the model yields nearly identical denoising velocity predictions in the subsequent step, regardless of the text prompts. Mathematically,this hypothesis can be describe as:

\[
\lim_{t \to 0} ({V}_{\text{}}({X}_{\text{t}},t,{C}_{\text{trg}})-{V}_{\text{}}({X}_{\text{t}},t,{C}_{\text{src}}))=0
\]

According to the above three hypothesis, we can infer the general cause of hyperparameter sensitive and the low editing flexibility. Due to the test-time-tuning process, We train the model to predict the velocity field V that satisfies the following equation:

\[
X_t-{V}_{\text{}}({X}_{\text{t}},t,{C}_{\text{src}})*t=X_0
\]

Therefore, due to Hypothesis 1, we can obtain the following equation:

\[
{X}_{\text{t2}}
={X}_{\text{init}}-{V}_{\text{}}({X}_{\text{init}},t_{init},{C}_{\text{src}})dt
\]
\[
{Y}_{\text{t2}}
={X}_{\text{init}}-{V}_{\text{}}({X}_{\text{init}},t_{init},{C}_{\text{trg}})dt
\]
\[
{Y}_{\text{t2}}-{X}_{\text{t2}}
=({V}_{\text{}}({X}_{\text{init}},t_{init},{C}_{\text{src}})-{V}_{\text{}}({X}_{\text{init}},t_{init},{C}_{\text{trg}}))dt
\]
\[
{X}_{\text{t1}}
={X}_{\text{t2}}-{V}_{\text{}}({X}_{\text{t2}},t_{2},{C}_{\text{src}})dt
\]
\[
{Y}_{\text{t1}}
={Y}_{\text{t2}}-{V}_{\text{}}({Y}_{\text{t2}},t_{2},{C}_{\text{trg}})dt
\]
\[
{Y}_{\text{t1}}-{X}_{\text{t1}}
=Y_{t2}-X_{t2}+({V}_{\text{}}({X}_{\text{t2}},t_{2},{C}_{\text{src}})-{V}_{\text{}}({Y}_{\text{t2}},t_{2},{C}_{\text{trg}}))dt
\]

Because flow-matching denoises in an almost linear manner and the $X_{init}$ is not a random noise,the latent representation $X_{t2}$ and $X_{t1}$ are almost at the low noise level,so we can approximately let $V(Xt2, t2, C_\text{src})=V(Xt2, t2, C_\text{src})$ due to the Hypothesis 3.

\[
{Y}_{\text{t1}}-{X}_{\text{t1}}
=Y_{t2}-X_{t2}+({V}_{\text{}}({X}_{\text{t2}},t_{2},{C}_{\text{src}})-{V}_{\text{}}({Y}_{\text{t2}},t_{2},{C}_{\text{src}}))dt
\]
Then we can apply the equatin in Hypothesis 1, getting:
\[
|{Y}_{\text{t1}}-{X}_{\text{t1}}|
<|{Y}_{\text{t2}}-{X}_{\text{t2}}|
\]
meaning although the difference in given prompt,the final output will be the same, limiting the editing flexibilty.
However, during the derivation process,there are two prerequisites that need to be met. Firstly, $|Y_{t2}-X_{t2}|$ need to smaller then the threshold $l$ defined in Hypothesis 1 and the value of l is strongly associated with the test-time-tuning steps. Secondly, $X_{t2}$ and $Y_{t2}$ should indeed in low noise level to Allow our approximation. And the noise level in $X_{t2}$ and $Y_{t2}$ are strongly associated with the noise level in $X_{init}$,the initial noise we gain in the inversion process of the reference video. In another words,if the two prerequisites are meet,the flow-matching process will mitigate the small errors and finally produce nearly the same video as the reference video. During the real training process ,we observed that the $l$ is too large. If the $X_t$ exceed l a little bit more, the model will generate videos that do not preserve the main feature in the reference video.

So far, we are able to generally explain why the model is too sensitive on initial noise $X_{init}$ and test-time-training steps.

To mitigate the sensitive issues,we propose a new training strategy aiming to decouple the relationship between TTT steps and $l$.Our method also reduce $l$ dramatically, reducing the stepwise changing issues.

We propose two solutions:

1)During training, we randomly replace the prompt of the reference video with the editing prompt. We gain the editing prompt by using gpt2 to produce background editing, subject editing and type editing text. Then we use the training free video editing methods(flow-edit) to gain the edited results as the ground truth. Although the ground truth is not accurate, it provides a guidance signal of the edited distribution, preventing all the velocity pointing at $X_0$.Due to the change of the ground truth, the $l$ is limited at a low level and has low relationship with the training step.

2)In hypothesis 2,we know that all edited videos reside in the vicinity of the reference video. We can simply add a certain level of normal-distribution noise to the ground truth $X_0$, letting
\[
X_0^*=X_0+\epsilon
\]
as the ground truth for the training goal.
Although the solution is fairly ordinary, in fact, this method constructs a mapping between distributions rather than a point-to-point mapping. During the test-time-tuning process,the model learns a mapping rule between the vicinity initial latent with noise and the distribution of all edited videos. The visual explanation can be seen in figure1.


Other concerns are why we choose a normal distribution instead of others.

According to the \textbf{Principle of Maximum Entropy}, When only partial knowledge about an unknown distribution is available, one should choose a probability distribution that aligns with this knowledge but has the maximum entropy.
Given the mean 
$x_{ij}^{\text{src}}$ and variance $\lambda^2$, the Gaussian distribution 
is the most unbiased choice for modeling uncertainty:
\begin{equation}
    x_{ij}^{\mathcal{F}} \sim \mathcal{N}(x_{ij}^{\text{src}}, \lambda^2)
\end{equation}
\end{comment}

%\begin{figure*}[t]
 %   \centering
  %  \includegraphics[width=0.8\textwidth]{fig/illustration.png}
  %  \caption{}
   % \label{fig:compare_visual}
   % \vspace{-10pt}
%\end{figure*}









%\begin{figure}[!htbp]
    %\centering
 %   \includegraphics[width=1\textwidth]{fig/Unet-comparison.jpg}
  %  \caption{Comparison with Tune A Video utilizing different training steps. As you can see, our training pipeline can generate similar objects and background when changing the Test-time-tuning steps. Tune A Video is cf to tuning steps and may deviate from the semantic information of the editing prompt when the tuning steps are high. The cartoon style jeep in 500 steps is an example of the bad case of overfitting. This figure shows that our methods are robust to hyperparameter.}
 %   \label{fig:visual}
%\end{figure}

\subsection{Contrastive Classifier-Free-Guidance: }
\label{subsec:contrastivecfg}
In~\cref{fig:toy} (F), after TDR, although the structure of the prior distribution is preserved, the generated points are still drawn closer to the source distribution trained in TTT. The same phenomenon occurs in video diffusion models: after TDR, the model no longer bypass $C_\text{src}$ and memorize the reference video entirely, yet the generated distribution still shifts toward the source distribution, showing a tendency of rendering the concepts introduced in the reference video.

To further cancel out the distribution shift and decouple the concepts of the source video which are planted into the model during training, we propose \textit{Contrastive Classifier-Free-Guidance}, an enhanced Classifier-Free-Guidance (CFG) which actively utilizes the source condition as a negative constraint.
The standard CFG~\cite{ho2022classifier} attempts to steer generation by creating a distribution shift between conditioned and unconditional predictions:
\begin{align}
    \hat{v}_\theta(x_t,t, C_{\text{trg}}) = v_\theta(x_t,t, C_{\text{neg}}) + \lambda\left( v_\theta(x_t,t, C_{\text{trg}}) - v_\theta(x_t,t, C_{\text{neg}}) \right)
\end{align}
where $C_{\text{neg}}$ is typically an empty or generic negative prompt, and $\lambda$ is the guidance scale. 
To further suppress the embedded optimization bias, we expand this guidance into a tri-directional formulation. We explicitly contrast the target against the source, establishing a semantic opposition between them, by introducing a secondary negative constraint leveraging the original source prompt $C_{\text{src}}$:
\begin{align}
    \hat{v}_\theta(x_t,t, C_{\text{trg}}) &= v_\theta(x_t,t, C_{\text{neg}}) + \lambda_1 \left( v_\theta(x_t,t, C_{\text{trg}}) - v_\theta(x_t,t, C_{\text{neg}}) \right) \nonumber \\&+ \lambda_2 \left( v_\theta(x_t,t, C_{\text{trg}}) - v_\theta(x_t,t, C_{\text{src}}) \right)
\end{align}
where $\lambda_1$ controls the standard unconditional guidance and $\lambda_2$ governs the strength of the semantic contrast between the source and target conditions.

By contrasting the two conditions, Contrastive CFG isolates and amplifies the semantic delta between them, repelling the sampling destination away from the source distribution. As demonstrated in~\cref{fig:toy}, applying standard CFG (G)—which merely pulls the velocity toward the target condition—yields only a marginal shift in the generated distribution due to the residual gravitational pull of the memorized source. In contrast, our Contrastive CFG (H) actively repels the generation process from the source concept. This active contrast guarantees crisp semantic transitions and fully restores the model's generative elasticity.


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/pca_comparison.jpg}
    \caption{PCA~\cite{hotelling1933analysis} visualization of the DiT latent representations. When TTT is applied without Async-NS, the representation blurs and the model fails to capture the reference video's structure. Async-NS enables the model to extract clear, aligned representation}
    \label{fig:spatial-entangle-visualize}
    \vspace{-4mm}
\end{figure}


\subsection{Asynchronous Noise Scheduling}
\label{subsec:asyncns}
While TDR and Contrastive CFG cure Conditioning Collapse, the fine-tuned network remains vulnerable to Spatial Entanglement. Because the tuned network learns to bypass the noisy input $x_t$ and directly memorize $x_0$, it fails to extract localized, semantically rich spatial representations. As visualized in~\cref{fig:spatial-entangle-visualize} (C), during inference, the representation becomes blurred and misaligned with the source video, with the foreground and background heavily entangled.


Many existing approaches attempt to alleviate Spatial Entanglement by modifying attention maps~\cite{kwon2024unified,zuo2025cut}, using pre-edited images as guide~\cite{ku2024anyvv,gao2025lora,liu2025stablev2v} or intervening the optimization phase with masks~\cite{gao2025lora,wang2025low}. However, these complicated methods often compromise the global structural coherence. In contrast, we propose \textit{Asynchronous Noise Scheduling} (Async-NS), an inference-time strategy that cleanly circumvents Spatial Entanglement by decoupling the integration trajectories of edited and anchored regions.





Our core insight is that temporal uniformity exacerbates Spatial Entanglement. Evaluating the entire latent at a single timestep $t$ allows the network to fall back on its memorized output. By explicitly assigning distinct noise levels and time embeddings to the edited versus anchored regions, we physically break the entanglement of representations. As evidenced in~\cref{fig:spatial-entangle-visualize} (B), this temporal asymmetry forces the network to process the regions distinctly, instantly restoring clear representational boundaries. Furthermore, this decoupling inherently aligns with the distinct generative needs of the regions: the edited area receives a high-noise regime ($T_\text{e}$) for the flexibility to render new concepts, while the preserved region is restricted to a low-noise regime ($T_\text{p}$) that carries the maximum information from the source video.

We define a frame-by-frame mask $M$, either from manual input for accuracy or from an automatic segmentation model for convenience, to mark the edited areas. $M$ is then downsampled to match the latent resolution and spatially smoothed into a continuous transition map $\tilde{M} \in [0, 1]$ to naturalize the concept boundaries in latent space. We define two asynchronous noise schedules: $\{t^i_\text{e}\}_{i=1}^N$ and $\{t^i_\text{p}\}_{i=1}^N$, with $t^N_{(\cdot)} = T_{(\cdot)}$ and $t^1_{(\cdot)} = 0$. The sampling starts from an initial latent $\hat{x}^N$, a noisy version of the source video latent with a mixed noise level, and at each step $i$, the asynchronous updates are spatially fused:
\begin{align}
\hat{x}^N &= \tilde{M}\odot x_{T_\text{e}} + (1-\tilde{M})\odot x_{T_\text{p}}\nonumber\\
\hat{x}^{i-1} &= \tilde{M} \odot \left( \hat{x}^i - \hat{v} \Delta t^{i}_\text{e} \right)+ (1 - \tilde{M}) \odot \left( \hat{x}^i - \hat{v} \Delta t^{i}_\text{p} \right)
\end{align}
where $\hat{v}$ denotes the final velocity by Contrastive CFG predicted with a spatially mixed timestep embedding of $t^i_\text{e}$ and $t^i_\text{p}$ as input: 
\begin{align}
    \hat{v}=\hat{v}_\theta(\hat{x}^i, t^i,C_\text{trg}),\quad t^i =\tilde{M}\odot t^i_\text{e}+(1-\tilde{M})\odot t^i_\text{p}
\end{align} 

By breaking the global temporal synchronization, Async-NS provides the model with a spatially clear, disentangled latent representation with distinct noise levels and timestep embeddings. Meanwhile, this formulation also grants the model localized freedom to aggressively overwrite target concepts along a longer integration path, while safely guiding unedited surroundings back to their exact physical state along a restricted, deterministic path.



\begin{comment}
The difference in noise level and timestep embeddings makes explicit distinctions among different regions, as shown in~\cref{fig:compare_visual}\C{TODO, change to visualization image} , also granting the model the localized latent freedom to aggressively overwrite target concepts along a longer integration path, while safely guiding unedited surroundings back to their exact physical state along a restricted, deterministic path.
\end{comment}
\begin{comment}
By implementing the Spatial-temporal representation learning in the last section, our model is able maintain the general moving trend. However the details in the reference videos are not totally preserved.
%We observed that it is hard for most of the previous methods to balance the motion loyalty and the alignment with the edited prompt. 

When we tend to significant change an object, other part of the video will experience unexpected change. This problem also exist in previous one-shot-tuning method. We find that this phenomenon is because of using a unified semantic similarity regularization hyperparameter globally. To solve this problem, we proposed a synchronous noise scheduling strategy in different semantic parts in a video.

Therefore, we introduce a synchronous noise scheduling strategy. In inference process, we start with an noisy latent gained from the reference video through inversion process. Our key concern is to apply different numbers of inversion steps in different areas on the original video. Fewer inversion steps mean more information are preserved in the noisy latent.

We first utilize a pretrained VLM to give a brief instruction of where to edit. To be more specific, given the original prompt of the input video, the edited prompt and one of the frames in the reference video, the VLM produce a word that refer to the area that need to be changed in the reference video. For example, if  the original prompt is "A jeep is moving on the road" and the target prompt is "A horse is running on the road", the VLM model will output a single word jeep. Then, the Grounded-SAM-2 will take this word as input and generate a mask on the reference video. Then, we down-sample this mask to latent space. We set two different noise levels for the masked and unmasked area. We also implement  linear transform in noise level at the edge of the masked area to achieve smooth edge transition. 

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{fig/async_noise_schedule.jpg}
    \caption{The visual description of our sementic mask and edited results.}
    \label{fig:compare_visual}
    \vspace{-10pt}
\end{figure*}
\end{comment}
\begin{comment}
To explicitly sever this conceptual tie and prevent the original appearance from dominating the edited area, we introduce Semantic Decoupling via a Contrastive CFG formulation. Rather than relying solely on a generic negative prompt, we actively utilize the original source prompt $C_{\text{src}}$ as a targeted negative constraint. We expand the velocity guidance equation into a tri-directional formulation:\begin{align}\hat{v}\theta(x_t, C{\text{trg}}) &= v_\theta(x_t, C_{\text{trg}}) + s_1 \cdot \left( v_\theta(x_t, C_{\text{trg}}) - v_\theta(x_t, C_{\text{neg}}) \right) \nonumber \&\quad + s_2 \cdot \left( v_\theta(x_t, C_{\text{trg}}) - v_\theta(x_t, C_{\text{src}}) \right)\end{align}where $s_1$ controls the standard unconditional guidance, and $s_2$ governs the strength of the semantic decoupling from the source concept.By leveraging this contrastive approach, we systematically disentangle the target generation from the source bias. The diffusion model is not only guided toward the user's desired target concept ($C_{\text{trg}}$), but is mathematically penalized for generating features associated with the original reference object ($C_{\text{src}}$). This final decoupling mechanism guarantees crisp, decisive semantic transitions, enabling the model to exhibit extreme editing flexibility while faithfully maintaining the underlying kinematic motion preserved by the optimization phase.

\begin{equation}
    \hat{\epsilon}_\theta(x_t, {C}_{\text{trg}}) = \epsilon_\theta(x_t, {C}_{\text{neg}}) + s \cdot \left( \epsilon_\theta(x_t, {C}_{\text{trg}}) - \epsilon_\theta(x_t, {C}_{\text{neg}}) \right)
\end{equation}

Too similar to the reference video at the edited area is need be avoid. Therefore, we adapt a similar solution just as we done to the negative prompt. This can be described as:

\begin{equation}
    \hat{\epsilon}_\theta(x_t, {C}_{\text{}}) = \epsilon_\theta(x_t, {C}_{\text{}}) + s_1 \cdot \left( \epsilon_\theta(x_t, {C}_{\text{}}) - \epsilon_\theta(x_t, {C}_{\text{neg}}) \right)+s_2 \cdot \left( \epsilon_\theta(x_t, {C}_{\text{}}) - \epsilon_\theta(x_t, {C}_{\text{src}}) \right)
\end{equation}

By leveraging this approach, our methods achieve a more flexible editing ability while maintaining the basic movement in the reference video.
\end{comment}


==> arxiv_meow-2/sec/5_experiment.tex <==
\section{Experiment}

\begin{table}[t]
  \caption{\textbf{Quantitative comparison with prior video editing approaches.} Best results are highlighted in \textcolor{red}{red}, and second-best in \textcolor{blue}{blue}. * refers that the method is re-implemented with our configurations.
  }
  
  \centering
  \label{tab:video_editing_comparison}

  \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{lccccccc}
    \toprule
    Methods &VBench$\uparrow$& CLIP-T$\uparrow$ & VEBench$\uparrow$&VQ$\uparrow$&IA$\uparrow$&SP$\uparrow$&OVL$\uparrow$ \\
    \midrule
    \multicolumn{8}{l}{\textit{Other Methods}} \\ 
     AnyV2V\cite{ku2024anyvv} & 4.80 &\textcolor{blue}{30.21} &0.53 &3.51&5.89&2.30&4.31\\
     Ground-A-Video\cite{jeong2024groundavideo} & 4.89 &28.51 &0.13&3.57&4.49&2.42& 3.90\\
     Token-flow\cite{geyer2024tokenflow} &4.82 &29.69 &\textcolor{blue}{0.67} &4.47&5.57&4.30&4.83\\
    
     Ditto \cite{bai2025ditto}& 4.88& 28.93&0.60&\textcolor{blue}{5.48}&5.95&3.32&\textcolor{blue}{5.62}\\
     Flow-align \cite{kim2026flowalign}& 4.93&27.72& 0.61&5.28&5.44&\textcolor{red}{7.23}&5.44\\
     Uniedit \cite{bai2025uniedit}&  4.31&\textcolor{red}{31.76} &0.64  &3.87&\textcolor{blue}{6.51}&0.54&5.04\\
      \midrule
    \multicolumn{8}{l}{\textit{Test-Time-Tuning Methods}} \\ 
    Tune-A-Video* \cite{wu2023tune}&\textcolor{red}{5.00}&28.40&0.72&5.34&6.15&3.63&5.39\\
    VidTTA*\cite{wang2025low}&\textcolor{blue}{4.98}&28.47&0.72&5.00&5.76&4.42&5.08\\
    \rowcolor{yellow!30}ElasticTTT&\textcolor{blue}{4.98}& 29.58&\textcolor{red}{0.72} &\textcolor{red}{6.19}&\textcolor{red}{7.50}&\textcolor{blue}{5.23}&\textcolor{red}{6.68} \\
  \bottomrule
  \end{tabular}
    \vspace{-3mm}
\end{table}



\subsection{Experiment setup}
To validate the effectiveness and robustness of ElasticTTT, we conducted extensive experiments and compared it with a wide range of video editing models. We utilize Wan2.1 1.3B~\cite{wan2025wan} as the base model and conduct TTT with Low Rank Adaptation (LoRA)~\cite{hu2022lora} for 100 steps. We set the TDR variance to $\sigma_\text{reg} = 0.2$, the CFG guidance scales to $\lambda_1=6, \lambda_2 = 2$, and distinct noise regimes to $T_\text{p}=0.55, T_\text{e}=0.97$. The segmentation mask $M$ is automatically generated by a segmentation model Grounded-SAM2~\cite{ravi2024sam2} with a VLM Qwen3-VL-32B~\cite{Qwen3-VL} to specify the edited concept.
All experiments are done on a single Nvidia pro6000 GPU, where our full method introduces only a $\sim$7\% inference-time overhead over vanilla TTT (approximately 5\% from Contrastive CFG and 2\% from Async-NS).
More implementation details, along with a sensitivity analysis on these hyperparameters that verifies the robustness of our method, are provided in Supplementary~\cref{exp}.
% \begin{comment}
% \subsection{Experiment setup}
% To validate the effectiveness and robustness of ElasticTTT, we conducted extensive experiments and compared them with a wide range of video editing models. We utilize Wan2.1 1.3B~\cite{wan2025wan} as the base model and conduct TTT with Low Rank Adaptation (LoRA)~\cite{hu2022lora} for 100 steps. We set the TDR variance to $\sigma_\text{reg} = 0.2$, the CFG guidance scales to $\lambda_1=6, \lambda_2 = 2$, and distinct noise regimes to $T_\text{p}=0.55, T_\text{e}=0.97$. The segmentation mask $M$ is automatically generated by a segmentation model Grounded-SAM2~\cite{ravi2024sam2} with a VLM Qwen3-VL-32B~\cite{Qwen3-VL} to specify the edited concept.
% All experiments are done on a single Nvidia pro6000 GPU. More details on the experiment setup are listed in Supplementary.
% We also conduct an ablation study on these hyperparameters to prove the stability.
% ElasticTTT remains highly efficient: it introduces only a $\sim$7\% inference-time overhead relative to the vanilla TTT baseline, of which approximately 5\% is attributed to Contrastive CFG and 2\% to the asynchronous noise scheduling strategy.
% \end{comment}
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{fig/qualitative_results.jpg}
    \caption{Visual comparisons with other methods. Our method strictly follows the editing instructions while successfully preserving the details in unedited regions.}
    \label{fig:qualitative_comparison}
    \vspace{-5mm}
\end{figure}

\subsubsection{Evaluation Datasets}
Prior works~\cite{ yang2025videograin,meral2024motionflow,kwon2024unified,liang2025looking,geyer2024tokenflow,liang2024flowvid} construct their testset by selecting text-video pairs from the Davis dataset~\cite{pont20172017,perazzi2016benchmark,caelles20182018}. However, either their data is not released~\cite{geyer2024tokenflow,kahatapitiya2024object} or the selection contains only limited editing tasktypes~\cite{liu2025stablev2v}. Thus, we choose to select a testset following the common protocol on our own, including 125 text-video pairs.
For comprehensive evaluation, our testset covers five different types of tasks, specifically: subject editing, background editing, subject addition, color adjustment, and general editing. We define general editing as reconstructing all visual elements in the video while preserving only the general motion dynamics of the reference subject. This editing mode is particularly valuable when the goal is to retain the cinematographic composition (or camera movement) rather than the visual content. We will release our selection to promote fair and comprehensive benchmarking for future works.




\subsubsection{Prior Methods}

We compare ElasticTTT against several strong video editing baselines: FlowAlign~\cite{kim2026flowalign}, UniEdit~\cite{bai2025uniedit}, Ditto~\cite{bai2025ditto}, VidTTA~\cite{wang2025low}, TokenFlow~\cite{geyer2024tokenflow}, AnyV2V~\cite{ku2024anyvv}, Tune-A-Video~\cite{wu2023tune} and Ground-A-Video~\cite{jeong2024groundavideo}. This selection represents a wide-range of conventional video editing paradigms, encompassing training-free methods~\cite{bai2025uniedit, geyer2024tokenflow, jeong2024groundavideo, kim2026flowalign}, first-frame-guided approaches~\cite{ku2024anyvv}, large-scale training-based models~\cite{bai2025ditto}, and other Test-Time Tuning (TTT) methods~\cite{wu2023tune, wang2025low}.
Notably, to ensure fair comparison with TTT-based baselines, we re-implement Tune-A-Video~\cite{wu2023tune} and VidTTA~\cite{wang2025low} using the \textit{exact same configurations} with ElasticTTT, including all settings of base model, training and inference.

\subsubsection{Evaluation Metrics}
We evaluate ElasticTTT and the baseline models using a comprehensive suite of objective and subjective metrics.

\emph{Automatic Metrics}.\ Following standard evaluation protocols~\cite{wang2025t3v2v,bai2025ditto, bai2025uniedit, wu2023tune}, we compute the CLIP similarity to measure semantic alignment between the edited video and the target prompt. In addition, we incorporate established metrics from video generation and editing benchmarks. We include metrics from VBench~\cite{huang2024vbench} to evaluate the overall visual quality and temporal consistency of the generated video. Specifically, we averaged 6 VBench metrics after normalizing them separately, to make a general assessment of the generated video. Also, we include the metric from VEBench~\cite{liu2025vebench} as a general indicator of video editing quality. These automatic metrics primarily serve as efficient and reproducible signals for model development, ablation analysis, and large-scale benchmarking.

\emph{Judge-Based Evaluation}.\ Despite their efficiency, traditional quantitative metrics often fail to capture nuanced editing requirements, such as fine-grained preservation in unedited regions or complex instruction adherence. To address this limitation, we leverage the advanced visual reasoning capabilities of a pretrained large Vision-Language Model (VLM). Specifically, we prompt GPT-5~\cite{openai2025gpt5systemcard} to evaluate generated videos along four dimensions: (1) Video Quality (VQ) measures the quality of generated video, independent of the source video and editing instructions; (2) Instruction Adherence (IA) measures the instruction-following ability of the editing prompt; (3) Source Video Preservation (SP) measures the preservation of the source video in unedited areas; (4) an overall score (OVL), for general assessment.

\emph{Human Study}.\ We further conduct a user study involving 10 participants, who independently rate each method along the same three dimensions: (1) Video Quality (VQ);  (2) Instruction Adherence (IA); and (3) Source preservation (SP). We averaged the three scores to obtain an overall human evaluation result for each video.
We randomly select one editing instruction for each video in our evaluation set to construct a subset for human evaluation. Participants are required to give a 1 to 5 rate on each criteria for each generated video. More details of evaluation metrics are shown in Supplementary~\cref{app:eval}.
%\ML{todo: check and update}

% We evaluate ElasticTTT and the baseline models using a comprehensive suite of objective and subjective metrics. Following standard evaluation protocols~\cite{}, we calculate CLIP similarity to measure the general semantic alignment between the output video and the editing prompt. Additionally, we incorporate established metrics from video generation and editing benchmarks, such as VBench and VEBench, to assess overall video quality and temporal consistency.

% However, traditional quantitative metrics often struggle to capture nuanced editing constraints, such as the preservation of fine details in unedited regions or complex instruction adherence. To overcome these limitations, we employ the advanced visual understanding capabilities of a pretrained large Vision-Language Model (VLM). Specifically, we prompt GPT-5~\cite{openai2025gpt5systemcard} to score the generated videos across four key dimensions: source video preservation, target instruction adherence, temporal consistency, and overall visual quality.


% \C{Unsure, maybe put into the results subsection.}
% We also conduct a subjective human evaluation, inviting [INSERT NUMBER] participants to rate the methods across the same dimensions. 

\begin{comment}
    

\begin{table}[t]
  \caption{\textbf{Quantitative comparison with prior video editing approaches.}$\uparrow$ means a higher score in this metric suggests a better performance. Best results are highlighted in \textcolor{red}{red}, and second-best in \textcolor{blue}{blue}. The yellow row refers to our ElasticTTT. The last four columns are scored by GPT-5.
  }
  \centering
  \label{tab:video_editing_comparison}
  \scriptsize
  \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{lccccccc}
    \toprule
    methods &VBench$\uparrow$& CLIP-T$\uparrow$ & VEBench$\uparrow$&VQ$\uparrow$&IA$\uparrow$&SP$\uparrow$&OVL$\uparrow$ \\
    \midrule
    \multicolumn{8}{l}{\textit{No Test-Time-Tuning}} \\ 
     AnyV2V & 4.80 &\textcolor{blue}{0.30} &0.53 &3.51&5.89&2.30&4.31\\
     Ground-A-Video & 4.89 &0.29 &0.13&3.57&4.49&2.42& 5.44\\
     Token-flow &4.82 &\textcolor{blue}{0.30} &\textcolor{blue}{0.67} &4.47&5.57&4.30&4.83\\
    
     Ditto & 4.88& 0.29&0.60&\textcolor{blue}{5.48}&5.95&3.32&\textcolor{blue}{5.62}\\
     Flow-align & \textcolor{blue}{4.93}&0.28& 0.61&5.28&5.44&\textcolor{red}{7.23}&5.44\\
     Uniedit &  4.31&\textcolor{red}{0.32} &0.64  &3.87&\textcolor{blue}{6.51}&0.54&5.04\\
      \midrule
    \multicolumn{8}{l}{\textit{Test-Time-Tuning Methods}} \\ 
    Tune-A-Video &5.00&0.28&0.72&5.34&6.15&3.63&5.39\\
    VidTTA&4.98&0.28&0.72&5.00&5.76&4.42&5.08\\
    \rowcolor{yellow!30}ElasticTTT&\textcolor{red}{4.98}& \textcolor{blue}{0.30}&\textcolor{red}{0.72} &\textcolor{red}{6.19}&\textcolor{red}{7.50}&\textcolor{blue}{5.23}&\textcolor{red}{6.68} \\
  \bottomrule
  \end{tabular}
\end{table}

\end{comment}





\subsection{Comparison with Previous Methods}
\begin{wraptable}[11]{R}{0.5\textwidth}
 \vspace{-30pt}
  \caption{\textbf{Human evaluation results}.Best results are highlighted in \textcolor{red}{red}, and second-best in \textcolor{blue}{blue}.
  }
  \label{tab:video_editing_comparison—human}
  \centering
  \renewcommand{\arraystretch}{1}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{lcccc}
    \toprule
    Methods & VQ $\uparrow$& IA $\uparrow$& SP $\uparrow$&Avg.$\uparrow$  \\
    \midrule
      
     AnyV2V~\cite{ku2024anyvv}  &2.50&2.61&2.48&2.54\\
     Ground-A-Video~\cite{jeong2024groundavideo} &1.95& 2.15 &2.37&2.16\\
     Token-flow~\cite{geyer2024tokenflow} &2.83& 2.63&3.16&2.87 \\
  
      
      Uniedit~\cite{bai2025uniedit} &2.36& 2.94&2.08 &2.46\\
         Ditto~\cite{bai2025ditto} &\textcolor{blue}{3.85}& \textcolor{blue}{3.20} &3.07 &3.37\\
      Flow-align~\cite{kim2026flowalign} &3.73&2.82&\textcolor{red}{3.81} &\textcolor{blue}{3.45}\\
     \rowcolor{yellow!30} ElasticTTT&\textcolor{red}{3.87}&\textcolor{red}{3.32}&\textcolor{blue}{3.61}&\textcolor{red}{3.60}  \\
    % p-score & 0.95& 0.81 &0.97& 0.625 \\
    
  \bottomrule
  \end{tabular}
\end{wraptable}

\cref{tab:video_editing_comparison} summarizes the quantitative comparison between ElasticTTT and competitive baseline methods. In general, TTT-based methods outperform prevailing video editing approaches due to their ability to adapt to the specific content and temporal dynamics of each input video at test time. Moreover, ElasticTTT achieves the strongest performance among TTT-based methods, with particularly substantial gains on VLM-based evaluations, which provide a holistic and fine-grained assessment of video editing quality across multiple dimensions (VQ 6.19, IA 7.50, and OVL 6.68). Although certain baselines match or exceed ElasticTTT on isolated metrics, they suffer from significant trade-offs. 

For example, Flow-align excels at preservation (SP 7.23) in unedited areas but struggles with editing elasticity and instruction adherence (IA 5.44). Conversely, Uniedit achieves strong semantic alignment with target instructions (evidenced by a high CLIP-T score of 31.76) but fails in preservation (SP 0.54), heavily distorting the original video. As shown in~\cref{fig:qualitative_comparison}, ElasticTTT achieves both precise editing adherence (ship and river, black stones) and source preservation (background building, rhino and trees), whereas other methods exhibit obvious compromises.

As shown in~\cref{tab:video_editing_comparison—human}, the results of human evaluation provide strong support for our quantitative findings. ElasticTTT achieves the highest performance (Average 3.60), indicating a clear human preference over the baseline methods. It excels particularly in editing adherence (IA 3.32) and achieves the top score for video quality (VQ 3.87). Even in preservation, where Flow-align peaks, ElasticTTT maintains a strong second-best performance (SP 3.61) without the severe trade-offs observed in competing models. Additionally, a study provided in the Supplementary~\cref{human} reveals a strong alignment between human volunteer scores and VLM evaluations, demonstrating the rationality of our VLM-based evaluation protocol.

\begin{wraptable}{r}[-1.5em]{0.5\textwidth}
  \centering
   % 视情况调整，消除上方空白
  \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{5pt}
 % \vspace{200pt}
  \caption{\textbf{Generalization to a larger base model.}Best results are highlighted in \textcolor{red}{red}.}
  \label{tab:model_scaling}
  \begin{tabular}{lcccc}
    \toprule
    Methods   & VQ$\uparrow$ & IA$\uparrow$ & SP$\uparrow$ & OVL$\uparrow$\\
    \midrule
    Wan2.2-5B-baseTTT & 5.05 & 5.09 & 4.40 & 4.91\\
    Wan2.2-5B-ours & \textcolor{red}{6.47} & \textcolor{red}{7.75} & 3.68 & \textcolor{red}{7.00}\\
    Wan2.1-1.3B-baseTTT & 5.34 & 6.15 & 3.63 & 5.39\\
    Wan2.1-1.3B-ours & {6.19} & {7.50} & \textcolor{red}{5.23} & 6.68\\
    \bottomrule
  \end{tabular}
   % 视情况调整，消除下方空白
\end{wraptable}

To examine whether ElasticTTT generalizes to larger base models, we further conduct the same experiment on Wan2.2-5B, comparing our full method against the vanilla TTT baseline under identical settings. As shown in \cref{tab:model_scaling}, ElasticTTT yields consistent and even more pronounced improvements on the larger backbone: it raises the overall score from 4.91 to 7.00 (+2.09), surpassing the corresponding gain observed on Wan2.1-1.3B (+1.29, from 5.39 to 6.68). The improvement is most evident in instruction adherence (IA 5.09 $\rightarrow$ 7.75) and video quality (VQ 5.05 $\rightarrow$ 6.47), indicating that our target distribution regularization and Contrastive CFG effectively unlock the richer generative prior of the larger model, which would otherwise be suppressed by TTT memorization. Notably, Wan2.2-5B equipped with ElasticTTT achieves the best overall score among all configurations (OVL 7.00), suggesting that our method scales favorably with model capacity. We observe a mild decrease in source preservation (SP 4.40 $\rightarrow$ 3.68), which we attribute to the stronger editing elasticity restored in the larger model: it follows editing instructions more aggressively, trading marginal preservation for substantially better semantic alignment—a trade-off that clearly pays off in the overall quality.



\subsection{Ablation Study}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/ablation_results.jpg}
    \caption{Visualized results of the ablation study.}
    \label{fig:ablation study}
    \vspace{-5mm}
\end{figure}
\begin{wraptable}{r}[-1.5em]{0.5\textwidth}
    \vspace{-10mm}
  \caption{\textbf{Quantitative results of the ablation study. }We exclude key components separately from the full model and report the resulting performance.Best results are highlighted in \textcolor{red}{red}. }
  
  \centering
  %   \scriptsize
  \renewcommand{\arraystretch}{1}
  \setlength{\tabcolsep}{5pt}
  %\vspace{-15pt}
  

  \label{tab:ablation}
  \begin{tabular}{lccccccc}
    \toprule
    Methods   & VQ$\uparrow$&IA$\uparrow$&SP$\uparrow$&OVL$\uparrow$\\
    \midrule
    None (baseline) &5.34&6.15&3.63&5.39\\
     w/o smooth transition &6.07&7.37&5.09&6.56\\
     w/o Async-NS&5.62&6.55&3.50&6.23\\
   
    w/o TDR  &6.13&7.45&5.36&6.64\\
    w/o contrastive CFG  &6.06&7.01&\textcolor{red}{5.64}&6.52\\
    \rowcolor{yellow!30}Full (ElasticTTT) &\textcolor{red}{6.19}&\textcolor{red}{7.50}&5.23&\textcolor{red}{6.68} \\
    
  \bottomrule
  \end{tabular}
\vspace{3mm}
\end{wraptable}


To assess individual contributions of our proposed designs, we conducted an ablation study systematically removing key components from the ElasticTTT pipeline. The results, presented both quantitatively in~\cref{tab:ablation} and qualitatively in~\cref{fig:ablation study}, confirm that the full method achieves the optimal balance across metrics, and also exhibits the best performance in~\cref{fig:ablation study}.



Omitting TDR negatively affects video quality, editing adherence, and overall score. Although removing it marginally improves the preservation score, this comes at the expense of the model's ability to execute complex edits. As shown in the first row in~\cref{fig:ablation study}, without TDR, the model merely reconstructs the source video and fails to add new concepts (wife, baby bear).

Removing Contrastive CFG leads to a noticeable decline in editing adherence and overall performance. 
Without this mechanism, the model struggles to fully follow the editing prompt, often resulting in an under-edited intermediate state between the reference and the target. As demonstrated in~\cref{fig:ablation study} (second row), the absence of Contrastive CFG results in subtle, less distinguishable edits that lack the visual clarity of our full method.

Both Async-NS and the additional smooth transitions are critical for cohesive video generation. Removing Async-NS causes a drop in all quantitative metrics. Qualitatively, as seen in the third row of~\cref{fig:ablation study}, without Async-NS the model loses its ability to accurately isolate the target regions, incorrectly modifying the foreground and background simultaneously. Meanwhile, using smooth transition map $\tilde{M}$ instead of $M$ is verified to be beneficial, as it results in a minor but distinct improvement in the overall score.
\begin{wraptable}{r}[-1.5em]{0.45\textwidth}
  \centering
  \vspace{-10pt}
  \caption{\textbf{Comparison between Async-NS and re-implemented Latent Blending under identical settings.} Best results are highlighted in \textcolor{red}{red}.}
  \label{tab:latent_blending}
  \begin{tabular}{lcccc}
    \toprule
    Methods   & VQ$\uparrow$ & IA$\uparrow$ & SP$\uparrow$ & OVL$\uparrow$\\
    \midrule
    Latent Blending & 4.65 & 6.02 & 1.08 & 4.71\\
    Async-NS & \textcolor{red}{6.19} & \textcolor{red}{7.50} & \textcolor{red}{5.23} & \textcolor{red}{6.68}\\
    \bottomrule
  \end{tabular}
  \vspace{-10pt}
\end{wraptable}
% \begin{bluehl}
We attribute this significant gap (OVL 6.68 vs. 4.71) to two primary factors.
First, Async-NS introduces \emph{asynchronous noise} inside the DiT forward process. By assigning different noise levels and timestep embeddings to the edited and preserved regions, it forms distinct regional representations during velocity prediction, thereby mitigating TTT-induced spatial entanglement. In contrast, post-hoc blending approaches only replace or mix latents after prediction, and thus cannot prevent entangled foreground/background features from being formed in the first place.

Second, such approaches rigidly hard-preserve the background, which proves counterproductive for realistic video editing: the unmasked region often requires soft physical adjustments, such as shadows, dust, boundary deformation, and contact effects. Forcibly stitching frozen background latents onto the edited content at mismatched noise levels produces visible seams and temporal artifacts, which explains the catastrophic preservation score of Latent Blending (SP 1.08) despite its seemingly conservative design. Async-NS instead suppresses spurious background drift while permitting these necessary interactions—a forward-pass desynchronization mechanism rather than a post-forward background replacement.

% \end{bluehl}





\begin{comment}
    
\emph{Async-NS} We conduct a two-stage ablation study. First, omitting the smooth transition introduces abrupt noise variations, failing to seamlessly connect edited and preserved areas, and degrading all metrics (Table \ref{tab:ablation}). Second, completely removing the strategy (using uniform initial noise) yields a better prompt alignment but destroys the structural details of the preserved regions, ultimately lowering the VLM and editing scores.



\emph{Contrastive CFG} 
Table \ref{tab:ablation} presents the ablation study in contrast Classifier-Free Guidance (CFG). Without it, the model struggles to fully follow the editing prompt, often resulting in an under-edited intermediate state between the reference and the target. Conversely, applying contrastive CFG enables more flexible editing, significantly improving semantic alignment and overall editing quality.

\emph{TDR} 
To validate the TDR, we conducted an ablation study (Table \ref{tab:ablation}). The results demonstrate that adding noise improves nearly all aspects of the generated video. Furthermore, applying this regularization strategy simultaneously improves both editing flexibility and overall visual quality.

\end{comment}


==> arxiv_meow-2/sec/6_conclusion.tex <==
\section{Conclusion}

In this paper, we present \textbf{ElasticTTT}, a novel Test-Time Tuning based video editing framework. We first analyze the prior collapse phenomenon brought by the inherent tension between the rigid optimization target in TTT and the generative nature of diffusion models. By introducing three novel techniques: Target Distribution Regularization, Contrastive CFG, and Asynchronous Noise Scheduling, we resolve the Conditioning Collapse and Spatial Entanglement issues caused by prior collapse and achieve SOTA performance on quantitative results and human evaluation. Detailed ablation studies quantify the contribution of each key component in our framework. We believe our work not only represents an important step toward more reliable diffusion-based models, but also highlights promising directions for designing better personalized AI systems.
